PRESTO: Progressive Pretraining Enhances Synthetic Chemistry Outcomes

Multimodal Large Language Models (MLLMs) have seen growing adoption across various scientific disciplines. These advancements encourage the investigation of molecule-text modeling within synthetic chemistry, a field dedicated to designing and conducting chemical reactions to synthesize new compounds with desired properties and applications. Current approaches, however, often neglect the critical role of multiple molecule graph interaction in understanding chemical reactions, leading to suboptimal performance in synthetic chemistry tasks. This study introduces PRESTO(Progressive Pretraining Enhances Synthetic Chemistry Outcomes), a new framework that bridges the molecule-text modality gap by integrating a comprehensive benchmark of pretraining strategies and dataset configurations. It progressively improves multimodal LLMs through cross-modal alignment and multi-graph understanding. Our extensive experiments demonstrate that PRESTO offers competitive results in downstream synthetic chemistry tasks. The code can be found at https://github.com/IDEA-XL/PRESTO.

==> sec/1-intro-new.tex <==
\section{Introduction}
% para1: multi-modal LM --> molecule-text modeling

% para2: molecule-text modeling --> under-perform on synthetic chemistry tasks, because of their disadvantage in multi-graph understanding, 

% para3: Scrutinizing into prior works \cite{}, we identify two main factors influencing multi-graph understanding ability: 1) pretraining strategy and 2) dataset configuration; 


% Para1: Deep learning for chemical reaction prediction has achieved many successes. They mostly use graph-based \cite{} or LM-based methods \cite{}. Recently, LM-based methods have drawn more attention due to the promising results when scaling up. 
Deep learning has revolutionized synthetic chemistry \citep{Zhou2017OptimizingCR, Liu2017RetrosyntheticRP, Granda2018ControllingAO, Mater2019DeepLI, Ucak2022RetrosyntheticRP, RXNFP} by precisely predicting, optimizing, and elucidating chemical reactions. Using extensive datasets of chemical structures and reaction conditions, it excels in forecasting products, designing molecules, and understanding reactivity principles.

% Para2: LM-based method for synthetic chemistry --> single-modal and multi-modal
Prior works have achieved extensive success in synthetic chemistry using LM-based methods~\citep{MolecularTransformer, YieldBERT, RXNFP}. However, these models mostly specialize in a few tasks of synthetic chemistry but struggle to generalize to other synthetic tasks. This is because they are pre-trained on domain-specific data, limiting their ability to share knowledge and adapt to new tasks of synthetic chemistry. To resolve the issue, multi-task methods \citep{T5Chem, Text+ChemT5, Chemformer} are explored and show a strong capability of handling tasks across domains. However, they are hindered by their dependence on sequential representation, disregarding molecular topology and structure.

% or ability to generalize to various chemistry tasks (\textit{e.g.}, reaction classification) was limited by a lack of shared chemical knowledge and adaptability issues. 
% For example, MolecularTransformer \citep{MolecularTransformer} is pre-trained on chemical reaction data, and cannot perform yield prediction; 

% issue1: multi-graph; 

% issue2: comprehensive evaluation; 

% issue3: incremental pre-training for adaptation on synthetic chemistry


% Para2: issues of existing methods: 1) single-task; 2) multi-task, but single-modality


% Para3: stepping into the LLM era. issue1: limited chemistry knowledge
Recently, researchers have turned to the off-the-shelf usage of general-purpose large language models (LLMs) \citep{ChatGPT, GPT4V, claude3} for chemistry tasks \citep{ChemBench, Jablonka2024LeveragingLL}. Despite pre-training on vast general corpora, these models face challenges in maintaining chemical plausibility \citep{ChemLLMBench, PromptEO}, demonstrating limited capabilities compared to task-specific deep learning models. 
% para-split: issue2: single-molecule understanding; 
% issue: prior work mostly focus on improving cross-modal alignment, or supervised fine-tuning, but hardly explores pretraining for multi-graph understanding and domain adaptation
\yuan{While prior methods \cite{MolCA, InstructMol, 3DMoLM, DrugChat, BioMedGPT} typically focus solely on aligning molecule representation with text or improving domain-adapted instruction-tuning processes, they overlook the crucial pre-training phase. }
% issue4: dataset configuration
Attempts to adapt general language models to chemistry, exemplified by \citep{Mol-Instruction, LLaSMol, ChemDFM}, primarily employ a text-only instruction-tuning approach, relying solely on supervised fine-tuning to perform synthesis-related tasks. In contrast, models such as \citep{MolCA, InstructMol, 3DMoLM} attempt to integrate multiple modalities into the textual space of language models and facilitate various tasks through instruction tuning. However, they are constrained by their focus on single-molecule understanding and lack robust training strategies and data set configurations, rendering them impractical for downstream applications. 

% Para4: 
% To address these limitations, a cross-domain model that harnesses language models' natural language understanding capabilities is critical to tackling versatile, multitask chemical reaction prediction tasks beyond simplistic sequential representations.
To effectively address the identified research gaps, we introduce \ModelName, a specialized framework tailored for chemical reaction tasks, harnessing the capabilities of multiple modalities LLMs across language and molecule. Our model supports interleaved molecule-text inputs as context, deepening the model's grasp of chemical reaction principles by effectively utilizing inter-relationships between molecule-molecule and molecule-text.
\yuan{InstructRXN has the following components:} 

\noindent % merge into above
\paragraph{Two-Stage Pre-training Strategy.} 
We comprehensively evaluate various pre-training strategies to achieve effective multi-graph understanding and adapt the LLM to the chemical reaction domain. After that, we propose a two-stage pre-training strategy that progressively cultivates the LM's ability of 1) cross-modal alignment and 2) multi-graph understanding and domain knowledge. Through extensive experiments, we demonstrate that our two-stage pre-training strategy can effectively cultivate an LLM's ability to multi-graph understanding and prepare the LLM's domain knowledge for later fine-tuning on chemical reaction tasks.
Supporting this, we construct a comprehensive pretraining dataset ($\sim$3M samples) comprising interleaved molecule-text data and name-conversion task data. We use synthetic procedure descriptions from the USPTO-Application corpus \citep{USPTO_patent} to identify molecular entities in text and convert them into 2D molecule graphs. Additionally, we introduce name conversion tasks for individual molecule graphs alongside text-only prediction tasks to deepen the model's understanding of molecule structures and representations. Empirical validation confirms that our pretraining dataset configuration allows the model to harness the intrinsic knowledge within chemical synthesis procedures effectively.

% issue: while chemical reaction prediction has been explored by prior LLM studies, they unfortunately encountered two issues of 1) 
% previous not cover all tasks of chemical reaction prediction
% not carefully design splitting, not consider data leakage issue
% ! draw a comparison table
\noindent
\paragraph{Comprehensive Chemical Reaction Benchmark for LLMs.} Previous approaches \citep{ChemLLM, Mol-Instruction, ChemDFM} mainly focus on constructing text-only SFT datasets, lacking relevance to chemical reaction tasks. We address these issues by integrating all relevant tasks into a multi-objective SFT dataset ($\sim$760k samples), supporting regression, classification, ranking, and generation tasks, spanning over scenarios including product prediction, retrosynthesis, reaction condition recommendation, and yielding prediction.
% paragraph-split
% lacking investigation into the training strategies
We compile a comprehensive evaluation suite across diverse synthesis scenarios, conduct meticulous data cleaning to prevent data leakage, and implement scaffold splitting to generate challenging test sets. These resources are utilized to examine targeted experiments exploring critical design aspects, including training procedures, model architecture ablation, dataset combinations, and scaling for training time and data. Through these comparative experiments, we rigorously validate the robustness of our framework and provide practical guidance for designing multi-modality LLMs in the chemical reaction domain.

% Our contributions can be summarized as follows:
% \begin{itemize}[leftmargin=*]
% \setlength{\itemsep}{0pt}
% \item Introducing \ModelName, a specialized framework for chemical reaction prediction, we integrate multiple molecule-text interleaved inputs as context to effectively understand and capture molecule-text relationships.
% \item Employing a triple-stage training strategy, we transition from a general-domain LLM to a domain expert. This advancement involves constructing a comprehensive pretraining dataset and enhancing instruction tuning by integrating relevant tasks into SFT samples.
% \item Developing a comprehensive evaluation suite across diverse synthesis scenarios, we explore various design aspects to identify open-source models with competitive performances across tasks, confirming their practical utility.
% \end{itemize}

Our contributions can be summarized as follows:
\begin{itemize}[leftmargin=*]
\setlength{\itemsep}{0pt}
\item Comprehensive evaluation of different training strategies
\item Given the experimental insight above, we propose a new two-stage training method that achieves state-of-the-art results among LLM-based methods.
\item Comprehensive benchmark for chemical reaction tasks: forward reaction prediction, reaction prediction, retrosynthesis prediction, reactant prediction, reagent recommendation, reaction type classification, and yielding regression.
% \item Developing a comprehensive evaluation suite across diverse synthesis scenarios, we explore various design aspects to identify open-source models with competitive performances across tasks, confirming their practical utility.
\end{itemize}

==> sec/1-intro.tex <==
\section{Introduction}

% Teaser: left:to theasks; right-up: SFT-data distribution; right-down: radar (3stages-all v.s. llama2)
% Para1: deep learning for chemical reaction prediction has achieved many successes
The integration of deep learning into the realm of synthetic chemistry \citep{Zhou2017OptimizingCR, Liu2017RetrosyntheticRP, Granda2018ControllingAO, Mater2019DeepLI, Ucak2022RetrosyntheticRP, RXNFP} has ushered in a paradigm shift, enabling precise prediction, optimization, and understanding of chemical reactions. Leveraging vast datasets encompassing chemical structures and reaction conditions, models excel in predicting reaction outcomes, facilitating molecule design, and unraveling fundamental principles underlying chemical reactivity.

% Para2: issues of existing methods: 1) single-task; 2) multi-task, but single-modality
Early efforts utilizing transformer-based models \citep{MolecularTransformer, YieldBERT, Chemformer} for chemistry tasks relied on pre-training in extensive domain-specific data. While proficient in specific reaction prediction tasks, their ability to generalize across various chemistry tasks was limited by a lack of shared chemical knowledge and adaptability issues. Although capable of handling tasks across domains, Multitask transformers like \citep{T5Chem, Text+ChemT5} are hindered by their dependence on sequential representation, disregarding molecular topology and structure.

% Para3: stepping into the LLM era. issue1: limited chemistry knowledge
Recently, researchers have turned to the off-the-shelf usage of general-purpose large language models (LLMs) \citep{ChatGPT, GPT4V, claude3} for chemistry tasks \citep{ChemBench, Jablonka2024LeveragingLL}. Despite pre-training on vast general corpora, these models face challenges in maintaining chemical plausibility \citep{ChemLLMBench, HatakeyamaSato2023PromptEO}, demonstrating limited capabilities compared to task-specific deep learning models. 
% para-split: issue2: single-molecule understanding; issue3: robust training; issue4: dataset configuration
Attempts to adapt general language models to chemistry, exemplified by \citep{Mol-Instruction, LLaSMol, ChemDFM}, primarily employ a text-only instruction-tuning approach, relying solely on supervised finetuning to perform synthesis-related tasks. In contrast, models such as \citep{MolCA, InstructMol, 3DMoLM} attempt to integrate multiple modalities into the textual space of language models and facilitate various tasks through instruction tuning. However, they are constrained by their focus on single-molecule understanding and lack robust training strategies and data set configurations, rendering them impractical for downstream applications. 

% Para4: 
% To address these limitations, a cross-domain model that harnesses language models' natural language understanding capabilities is critical to tackling versatile, multitask chemical reaction prediction tasks beyond simplistic sequential representations.
To effectively address the identified research gaps, we introduce \PipeName{}, a specialized framework tailored for chemical reaction tasks, harnessing the capabilities of multiple modalities LLMs across language and molecule. Our model supports interleaved molecule-text inputs as context, deepening the model's grasp of chemical reaction principles by effectively utilizing inter-relationships between molecule-molecule and molecule-text.
\yuan{InstructRXN has the following three components:} 

\noindent
\paragraph{Triple-Stage Training Strategy.} 
% We propose a triple-stage training strategy that progressively cultivates the LM's ability of 1) cross-modal alignment; 2) multi-graph understanding, and domain knowledge; 3) downstream adaptation; 
% % align: inject mol repr to general LLM textual space
% pre-train: shift to chemistry synthetic procedure domain corpus + adapt to interleaved input format
% SFT: adapt to downstream chemical reaction prediction tasks
We introduce a comprehensive triple-stage training strategy comprising alignment, pre-training, and supervised finetuning (SFT). 
While prior methods \cite{MolCA, InstructMol, 3DMoLM, DrugChat, BioMedGPT} typically focus solely on aligning molecule representation with text or improving domain-adapted instruction-tuning processes, they overlook the crucial pre-training phase. 
Through extensive experimentation, we demonstrate that our triple-stage setup facilitates a smoother transition of a general-domain LLM to a model capable of accommodating external modalities and effectively completing specialized chemical reaction tasks.
\noindent
\paragraph{Dataset Construction in Pretraining Stage.} We construct a comprehensive pretraining dataset ($\sim$3M samples) comprising molecule-text interleaved data and name-conversion task data. We use synthetic procedure descriptions from the USPTO-Application corpus \citep{USPTO_patent} to identify molecular entities in text and convert them into 2D molecule graphs. Additionally, we introduce name conversion tasks for individual molecule graphs alongside text-only prediction tasks to deepen the model's understanding of molecule structures and representations. Empirical validation confirms that our pretraining dataset configuration allows the model to harness the intrinsic knowledge within chemical synthesis procedures effectively.

\noindent
\paragraph{Instruction Tuning Enhancement.} Previous approaches \citep{ChemLLM, Mol-Instruction, ChemDFM} mainly focus on constructing text-only SFT datasets, lacking relevance to chemical reaction tasks. We address these issues by integrating all relevant tasks into a multi-objective SFT dataset ($\sim$760k samples), supporting regression, classification, ranking, and generation tasks, spanning over scenarios including product prediction, retrosynthesis, reaction condition recommendation, and yielding prediction.

\noindent
\paragraph{Framework Validation.} We compile a comprehensive evaluation suite across diverse synthesis scenarios, conduct meticulous data cleaning to prevent data leakage, and implement scaffold splitting to generate challenging test sets. These resources are utilized to examine targeted experiments exploring critical design aspects, including training procedures, model architecture ablation, dataset combinations, and scaling for training time and data. Through these comparative experiments, we rigorously validate the robustness of our framework and provide practical guidance for designing multi-modality LLMs in the chemical reaction domain.

% Our contributions can be summarized as follows:
% \begin{itemize}[leftmargin=*]
% \setlength{\itemsep}{0pt}
% \item Introducing \ModelName, a specialized framework for chemical reaction prediction, we integrate multiple molecule-text interleaved inputs as context to effectively understand and capture molecule-text relationships.
% \item Employing a triple-stage training strategy, we transition from a general-domain LLM to a domain expert. This advancement involves constructing a comprehensive pretraining dataset and enhancing instruction tuning by integrating relevant tasks into SFT samples.
% \item Developing a comprehensive evaluation suite across diverse synthesis scenarios, we explore various design aspects to identify open-source models with competitive performances across tasks, confirming their practical utility.
% \end{itemize}
